Benchmarking air-conditioning energy performance of residential rooms based on regression and clustering techniques

Air conditioning (AC) accounts for a critical portion of the global energy consumption. To improve its energy performance, it is important to fairly benchmark its energy performance and provide the evaluation feedback to users. However, this task has not been well tackled in the residential sector. In this paper, we propose a data-driven approach to fairly benchmark the AC energy performance of residential rooms. First, regression model is built for each benchmarked room so that its power consumption can be predicted given different weather conditions and AC settings. Then, all the rooms are clustered based on their areas and usual AC temperature set points. Lastly, within each cluster, rooms are benchmarked based on their predicted power consumption under uniform weather conditions and AC settings. A real-world case study was conducted with data collected from 44 residential rooms. Results show that the constructed regression models have an average prediction accuracy of 85.1% in cross-validation tests, and support vector regression with Gaussian kernel is the overall most suitable model structure for building the regression model. In the clustering step, 44 rooms are successfully clustered into seven clusters. By comparing the benchmarking scores generated by the proposed approach with two sets of scores computed from historical power consumption data, we demonstrate that the proposed approach is able to eliminate the influences of room areas, weather conditions, and AC settings on the benchmarking results. Therefore, the proposed benchmarking approach is valid and fair. As a by-product, the approach is also shown to be useful to investigate how room areas, weather conditions, and AC settings affect the AC power consumption of rooms in real life.

==> temp_txt <==

\nomenclature[A]{$AC$}{air conditioning}
\nomenclature[A]{$ACS$}{air conditioning system}
\nomenclature[A]{$EPI$}{energy performance index}
\nomenclature[A]{$EPS$}{energy performance score}
\nomenclature[A]{$IEA$}{International Energy Agency}
\nomenclature[A]{$SUTD$}{Singapore University of Technology and Design}
\nomenclature[A]{$EER$}{energy efficiency ratio}

\nomenclature[V]{$C_r$}{overall thermal capacity of the cooled room
  \nomunit{$\mathrm{J/\,^{\circ}C}$}}
\nomenclature[V]{$T_r$}{room temperature
    \nomunit{$\mathrm{\,^{\circ}C}$}}
\nomenclature[V]{$\dot{Q}_{ac}$}{rate of heat loss through the AC system
    \nomunit{$\mathrm{W}$}}
\nomenclature[V]{$R_w$}{thermal resistance of the wall
  \nomunit{$\mathrm{\,^{\circ}C/W}$}}
\nomenclature[V]{$T_a$}{ambient air temperature
    \nomunit{$\mathrm{\,^{\circ}C}$}}
\nomenclature[V]{$\dot{Q}_{sun}$}{rate of heat gain from solar radiation
    \nomunit{$\mathrm{W}$}}
\nomenclature[V]{$\dot{Q}_{hum}$}{rate of heat gain from human activities
  \nomunit{$\mathrm{W}$}}

\nomenclature[V]{$\Delta T_r$}{change of room temperature
    \nomunit{$\mathrm{\,^{\circ}C}$}}
\nomenclature[V]{$Q_{ac}$}{total heat loss through the AC system
    \nomunit{$\mathrm{J}$}}
\nomenclature[V]{$\bar{T}_a$}{average room temperature
  \nomunit{$\mathrm{\,^{\circ}C}$}}
\nomenclature[V]{$\bar{T}_r$}{average ambient temperature
    \nomunit{$\mathrm{\,^{\circ}C}$}}
\nomenclature[V]{$t_{seg}$}{duration of one AC operation segment
    \nomunit{$\mathrm{s}$}}
\nomenclature[V]{$Q_{sun}$}{heat grain from solar radiation
  \nomunit{$\mathrm{J}$}}
\nomenclature[V]{$Q_{hum}$}{heat gain from human activities
    \nomunit{$\mathrm{J}$}}

\nomenclature[V]{$C_a$}{specific heat capacity of air
    \nomunit{$\mathrm{J/(kg\,^{\circ}C)}$}}
\nomenclature[V]{$\rho_a$}{density of air
  \nomunit{$\mathrm{kg/m^3}$}}
\nomenclature[V]{$H_r$}{room height
    \nomunit{$\mathrm{m}$}}
\nomenclature[V]{$A_r$}{room area
    \nomunit{$\mathrm{m^2}$}}
\nomenclature[V]{$U_w$}{wall thickness
    \nomunit{$\mathrm{m}$}}
\nomenclature[V]{$k_w$}{thermal conductivity of the wall
    \nomunit{$\mathrm{W/ m\,^{\circ}C}$}}
\nomenclature[V]{$A_w$}{wall area
    \nomunit{$\mathrm{m^2}$}}

\nomenclature[V]{$T_{set}$}{temperature set point
    \nomunit{$\mathrm{\,^{\circ}C}$}}
\nomenclature[V]{$T_{ri}$}{initial room temperature
    \nomunit{$\mathrm{\,^{\circ}C}$}}

\nomenclature[V]{$EER_o$}{overall energy efficiency ratior of the AC system
    \nomunit{}}
\nomenclature[V]{$\bar{p}_{ac}$}{average power consumed by the AC system
    \nomunit{$\mathrm{W}$}}

\nomenclature[V]{$C_{s2h}$}{overall conversion ratio from solar radiation to heat
    \nomunit{}}
\nomenclature[V]{$\bar{p}_{si}$}{average solar irradiance
    \nomunit{$\mathrm{W}$}}

